Expansive Supervision for Neural Radiance Field

Neural Radiance Field (NeRF) has achieved remarkable success in creating immersive media representations through its exceptional reconstruction capabilities. However, the computational demands of dense forward passes and volume rendering during training continue to challenge its real-world applications. In this paper, we introduce Expansive Supervision to reduce time and memory costs during NeRF training from the perspective of partial ray selection for supervision. Specifically, we observe that training errors exhibit a long-tail distribution correlated with image content. Based on this observation, our method selectively renders a small but crucial subset of pixels and expands their values to estimate errors across the entire area for each iteration. Compared to conventional supervision, our approach effectively bypasses redundant rendering processes, resulting in substantial reductions in both time and memory consumption. Experimental results demonstrate that integrating Expansive Supervision within existing state-of-the-art acceleration frameworks achieves 52% memory savings and 16% time savings while maintaining comparable visual quality.

==> content/2-related.tex <==



\section{Related Work}




\subsection{Neural Radiance Field}


Neural radiance field~\cite{nerf} has revolutionized the field of 3D computer vision by leveraging multilayer perceptrons (MLPs) to implicitly represent the radiance field. Its outstanding performance in 3D reconstruction and novel view synthesis has inspired a plethora of research~\cite{mipnerf,mipnerf360,mm-mirror,mm-pi,mm-re,mm-ff}. In terms of rendering quality, several works have focused on addressing aliasing artifacts and improving multi-scale representation. Examples of such works include Mip-NeRF~\cite{mipnerf}, Zip-NeRF~\cite{zipnerf}, and Tri-MipRF~\cite{trimiprf}.
For the adaption of NeRF to unbounded $360^\circ$ scenes, several methods have implemented foreground-background separation and non-linear scene parameterization to optimize the realism of the scenes ($e.g.$ NeRF++~\cite{nerfplusplus}, Mip-NeRF360~\cite{mipnerf360}).
As a novel representation of 3D media content, NeRF has also sparked significant interest in various downstream applications, including segmentation~\cite{nerf-seg-1,nerf-seg-2,nerf-seg-3}, editing~\cite{edit-1,edit-2,edit-3,edit-4,edit-5}, and generation~\cite{gen-1,gen-2,gen-3,gen-4,gen-5}.


\subsection{Efficient Training for NeRF}
NeRFs have been challenged by the time-consuming training and rendering, primarily due to the intensive computation involved in volume rendering.
Although recent advancements have enabled real-time rendering of NeRFs on mobile devices~\cite{mobile-r2l}, the training process still demands a significant amount of time and effort.
In order to accelerate training, various methods have been proposed. One of effective way is storing view-independent features in an explicit representation, which trades speed for space. 
Efficient explicit representations include octrees~\cite{nsvf, plenoctree}, point cloud~\cite{pointnerf}, voxel grids~\cite{dvgo, plenoxel}, low rank tensors~\cite{tensorf} and hash tables~\cite{ingp}. 
Another line of research focuses on employing decomposition schemes to reduce latency, such as DoNeRF~\cite{donerf} and KiloNeRF~\cite{kilo}.

The key distinction between existing acceleration techniques~\cite{derf,fastnerf,tensorf,ingp,strivec,mobilenerf,merf} and our method lies in the elimination of costly renderings. While existing methods primarily focus on reducing computation for each rendering pixel, our method addresses the issue from a supervisory perspective by reducing the number of rendering pixels required. To the best of our knowledge, our method is the first to achieve NeRF training acceleration through partial supervision. % offering additional benefits in terms of memory efficiency and adaptability.




